Defending Against Intelligent Attackers at Large Scales

We investigate the scale of attack and defense mathematically in the context of AI's possible effect on cybersecurity. For a given target today, highly scaled cyber attacks such as from worms or botnets typically all fail or all succeed. Here, we consider the effect of scale if those attack agents were intelligent and creative enough to act independently such that each attack attempt was different from the others or such that attackers could learn from their successes and failures. We find that small increases in the number or quality of defenses can compensate for exponential increases in the number of independent attacks and for exponential speedups.

==> graveyard.tex <==
calculate how much the likelihood of breach ($L$) is affected by changes in both the number of defenses ($n$) and the number of attacks ($N$) in equation \ref{partial_L}. 

\begin{subequations}
\label{partial_L}
\begin{gather}
    \frac{\partial L}{\partial N} = -(1-p^{n})^{N}ln(1-p^{n}) \label{partial_L_N} \\
    \frac{\partial L}{\partial n} = Np^{n}ln(p)(1-p^{n})^{N-1} \label{partial_L_n}
\end{gather}
\end{subequations}

Balancing these two rates, we can evaluate how much AI needs to scale up defenses to keep pace with an increased number of attacks as in equations \ref{Rn_RN} and \ref{Rn_RN_approx}. 

\begin{subequations}
\label{Rn_RN}
\begin{gather}
    \frac{\Delta_{N}}{\Delta_{n}} = -\frac{\partial L / \partial n}{\partial L / \partial N}  \\
    \frac{\Delta_{N}}{\Delta_{n}} = \frac{Np^{n}ln(p)}{(1-p^{n})ln(1-p^{n})}
\end{gather}
\end{subequations}

Equation \ref{Rn_RN} can be simplified by a few approximations based on $p^n$ being small (note that $0.5^{10}$ is less than $10^{-3}$). Firstly, $ln(1-p^{n}) \approx -p^{n}$, and secondly, $(1-p^{n}) \approx 1$. Those approximations lead to equation \ref{Nnrate} which can be integrated to give equation \ref{Nexponential}.

\begin{subequations}
\label{Rn_RN_approx}
\begin{gather}
    \label{Nnrate}
    \frac{\Delta_{N}}{\Delta_{n}} \approx -Nln(p)  \\
    \label{Nexponential}
    N = N_{o}e^{-nln(p)}
\end{gather}
\end{subequations}





\begin{subequations}
\label{L_s_n}
\begin{gather}
    \label{L_s_full}
    \partial L / \partial s = -ln(1-e^{-\lambda \tau}) N_{a} \frac{T}{\tau} e^{-\lambda \tau} (1-L) \\
    \partial L / \partial n = -s\lambda \tau \frac{e^{-\lambda \tau n}}{1-e^{-\lambda \tau n}} N_{a}\frac{T}{\tau}e^{-\lambda \tau} (1-L) \\
\end{gather}
\end{subequations}

\begin{subequations}
\label{s_N}
\begin{gather}
    \Delta_{n} / \Delta_{s} \approx \frac{1}{s\lambda \tau} \\
    s = N_{o} e^{\lambda \tau n} \\
    N_{o} = -\frac{ln(1-L{o})}{N_{a} \frac{T}{\tau}e^{-\lambda \tau}}
\end{gather}
\end{subequations}



Mathematically, the sensitivity of likelihood of breach ($L$) to imbalances in defense to offense speed ratios ($\lambda \tau$) is given equation \ref{eqnLlamtau}, where the two variables $\lambda$ and $\tau$ are treated as a single variable representing the relative speed of defense compared to offense. Equation \ref{eqnLlamtau} is always negative because increases in $\lambda \tau$ always improve defense and drive down the likelihood of breach. 

\begin{equation}
    \label{eqnLlamtau}
    \partial L / \partial (\lambda \tau) = -N n e^{-\lambda \tau n} (1 - e^{-\lambda \tau n})^{N-1} 
\end{equation}




These equations are structurally identical to eqn =\ref{blockade_equation}: $L=1-(1-p^{n})^{N}$, describing the basic blockade defense. In the blockade equation \ref{blockade_equation}, the probability of bypassing a defense ($p$) was raised to the number of defenses ($n$). In this combined Blockade and Delay case, it is the likelihood of not detecting an attack attempt ($u$) that is raised to some multiple of the number of defenses ($n$), either $2$ or $(1-p)/p$. That multiple makes the exponential value of adding defenses even stronger in this case than in the pure blockade strategy, even in the pessimistic case where defenders are certain to defeat defenses in their second attempt. If the defenses are so weak that attackers are likely to defeat them in their first attempt, $(1-p)/p < 1$, then adding defenses still provides exponential advantage as compared to adding attackers, but at a slower rate than in the pure blockade strategy.

